PokeGym: Mastering Long-Horizon, Open-World 3D Games via Graph-Guided Multimodal Evolution

Mastering long-horizon, vision-only 3D games requires agents to improve from experience across consecutive attempts while coordinating perception, strategy, and action. We introduce PokeGym, a benchmark built upon Pok\'emon Legends: Z-A, comprising 114 navigation, interaction, and target-localization tasks in dense, dynamic urban scenes. PokeGym evaluates test-time improvement across repeated attempts at the same task without exposing game states to the agent. To master PokeGym, we propose GraphEvo, a graph-guided multimodal test-time learning framework that jointly evolves visual enhancements, language strategies, and action macros while keeping the agent backbone frozen. A cross-modal graph predictor estimates the performance of newly generated configurations, and a disagreement-aware selector chooses candidates for execution, enabling efficient search in an open-ended configuration space without exhaustive rollouts. GraphEvo achieves a 60.18% average success rate on PokeGym, outperforming the strongest baseline by over 6%. Ablations demonstrate the contributions of visual adaptation, cross-modal modeling, and graph-guided selection, while experiments on ALFRED show transfer to household tasks.

==> arxiv-peramble.tex <==
\def\eg{\emph{e.g.~}} \def\Eg{\emph{E.g.~}}
\def\ie{\emph{i.e.~}} \def\Ie{\emph{I.e.~}}
\def\cf{\emph{cf.~}} \def\Cf{\emph{Cf.~}}
\def\etc{\emph{etc.~}} \def\vs{\emph{vs.~}}
\def\wrt{w.r.t.~} \def\dof{d.o.f.~}
\def\iid{i.i.d.~} \def\wolog{w.l.o.g.~}
\def\etal{\emph{et al.~}}

\usepackage[T1]{fontenc}
\usepackage{amssymb}   % 提供对勾符号 \checkmark
% \usepackage{textcomp}   % 提供直引号 \textquotedbl

\usepackage{graphicx}
\usepackage{tabularx}  % 自动调整列宽
\usepackage{makecell}  % 支持表头换行
\usepackage{multirow}   % 处理多行合并
\usepackage{graphicx}   % 用于调整表格宽度 \resizebox
\usepackage{colortbl} % 用于表格行/列染色
\usepackage{xcolor}
%\usepackage[table]{xcolor}   % 提供 \rowcolor 等表格颜色命令
%\usepackage{orcidlink}
\usepackage{amsmath}
%\usepackage{cleveref}
\usepackage{url}
\usepackage{enumitem}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{booktabs}
\usepackage{tcolorbox}
\tcbuselibrary{breakable}  % 允许 promptbox 跨页
\usepackage{caption}    % 让 strip 内也能用 \caption
%\usepackage[fixfootnote]{cuted}     % 提供 strip 环境
\usepackage{etoolbox}     % 用于全局环境钩子



\definecolor{za-pink}{rgb}{0.79, 0.62, 0.70}
\definecolor{za-grey}{rgb}{0.43, 0.45, 0.48}
\definecolor{za-dark}{rgb}{0.19, 0.16, 0.12}
\definecolor{za-green}{rgb}{0.25, 0.71, 0.48}

%\newcommand{\pokeza}{\textbf{\textcolor{za-pink}{Pokémon} \textcolor{za-grey}{Legends}:~\textcolor{za-dark}{Z}-\textcolor{za-green}{A}}}

\newcommand{\pokeza}{\textbf{\textcolor{black}{Pokémon} \textcolor{black}{Legends}:~\textcolor{black}{Z}-\textcolor{black}{A}}}

\newcommand{\no}{$\times$}
\newcommand{\yes}{\checkmark}





% 自定义一个叫 promptbox 的环境
\newtcolorbox{promptbox}[1][]{
	colback=yellow!15!white,   % 背景色：更饱和的浅黄色
	colframe=yellow!90!black, % 边框色：更亮的黄色
	fonttitle=\bfseries,    % 标题字体加粗
	title=#1,               % 允许传入标题
	boxrule=0.5mm,          % 边框粗细
	arc=2mm,                % 圆角弧度
	before upper={\setlength{\parskip}{0pt}\setlength{\parindent}{0pt}\small},
	left=2mm, right=2mm, top=2mm, bottom=2mm % 内边距
}
% 定义高亮颜色
\definecolor{highlightgray}{gray}{0.9}



%\usepackage{marvosym}
%\newcommand{\corresponding}{\texorpdfstring{$^{\textrm{\Letter}}$}{}}
%\usepackage{cuted} 

%\newlength{\IEEEteaserwidth}
%\setlength{\IEEEteaserwidth}{\dimexpr2\columnwidth+\columnsep\relax}

==> emoji.tex <==
\usepackage{stringenc}
\usepackage{hwemoji} % 原始QA没有提到这个，但很重要

% ref https://tex.stackexchange.com/questions/268069/how-do-i-enter-an-arbitrary-unicode-code-point-with-pdftex#329835

\newcommand*{\uni}{}
\DeclareRobustCommand*{\uni}[1]{%
  \begingroup
    \StringEncodingConvert\x{%
      \pdfunescapehex{%
        00%
        \ifnum"#1<"100000 0\fi
        \ifnum"#1<"10000 0\fi
        \ifnum"#1<"1000 0\fi
        \ifnum"#1<"100 0\fi
        \ifnum"#1<"10 0\fi
        #1%
      }%
    }{utf32be}{utf8}%
    \everyeof{\noexpand}%
    \endlinechar=-1 %
  \edef\x{%
    \endgroup
    \scantokens\expandafter{%
      \expandafter\unexpanded\expandafter{\x}%
    }%
  }\x
}

%\usepackage[pdfencoding=auto]{hyperref}
\pdfstringdefDisableCommands{%
  \def\uni#1{\unichar{"#1}}%
}

==> figs/Correlation_Heatmap.tex <==
\begin{figure*}[t]
	\centering
	% 请根据实际文件名替换
	\includegraphics[width=0.9\textwidth]{res/Correlation_Heatmap.pdf} 
	\caption{Cross-Benchmark Pearson Correlation Matrix. 
		}
	\label{fig:corr_heatmap}
\end{figure*}

==> figs/Correlation_LineChart.tex <==
\begin{figure*}[t]
	\centering
	% 请根据实际文件名替换
	\includegraphics[width=1.0\textwidth]{res/Correlation_LineChart.pdf}
	\caption{Correlation Trends across External Benchmarks.
		The line chart traces the Pearson correlation coefficients ($r$) of selected PokeGym categories across diverse external benchmarks. 
		}
	\label{fig:corr_profile}
\end{figure*}

==> figs/Correlation_Scatter.tex <==
\begin{figure*}[t]
	\centering
	% 请根据实际文件名替换
	\includegraphics[width=1.0\textwidth]{res/Correlation_Scatter.pdf}
	\caption{Cross-Domain Pearson Correlation Analysis. 
		Scatter plots displaying the relationship between specific PokeGym tasks and external benchmarks. 
		Each data point represents an evaluated VLM. 
		The dashed lines indicate the linear regression fit with 95\% confidence intervals (shaded regions). 
		}
	\label{fig:corr_scatter}
\end{figure*}

==> figs/all.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{res/all.pdf}
    % \caption{Overview of PokeGym and GraphEvo. \textbf{Top:} PokeGym is a 3D vision-only benchmark for evaluating test-time learning through iterative multimodal evolution. \textbf{Bottom:} GraphEvo jointly evolves visual, language, and action modalities and models their cross-modal synergy via a GNN.}
    \caption{Overview of PokeGym and GraphEvo. \textbf{Top:} PokeGym is a 3D vision-only benchmark for evaluating test-time learning through iterative multimodal evolution. \textbf{Bottom:} in contrast to isolated single-modality evolution (a), GraphEvo evolves the visual, language, and action modalities jointly and models their cross-modal synergy via a GNN (b); the evolved candidates are further scored and selected by the performance predictor and the disagreement-aware selector (Fig.~\ref{fig:framework}).}
    \label{fig:all}
\end{figure*}


==> figs/behavior.tex <==
\begin{figure*}[htbp] % [t] 表示优先将图片放在页首，也可以用 [htbp] 让系统自动调整
	\centering
	% width=\textwidth 确保图片宽度占满正文宽度
	\includegraphics[width=\linewidth]{figs/faceted_bar_behavioral.pdf} 
	
	\caption{\textbf{Behavioral Analysis of Successful and Failed Episodes.} 
    Metrics: Ineffective Move Rate (\textbf{IM\%}: the percentage of decision steps with movement actions that resulted in no spatial displacement), Recovery Rate (\textbf{Rec\%}: percentage of non-IMs immediately following an IM), Maximum Consecutive Ineffective Moves (\textbf{MaxIM}), and Action Entropy (\textbf{Ent}: the Shannon entropy of actions during $\ge 3$ consecutive ineffective moves).}
	\label{fig:behavior}
\end{figure*}

==> figs/complex.tex <==
\begin{figure*}[htbp]
    \centering
    % 请将 'environmental_complexity.png' 替换为你实际的图片文件名
    \includegraphics[width=0.6\textwidth]{res/complex.pdf} 
    \caption{Environmental Complexity in PokeGym. Qualitative examples of diverse challenges across five key dimensions.}
    \label{fig:env_complexity}
\end{figure*}

==> figs/correlation.tex <==
\begin{figure}[t] % [t] 表示优先将图片放在页首，也可以用 [htbp] 让系统自动调整
	\centering
	% width=\textwidth 确保图片宽度占满正文宽度
	\includegraphics[width=\linewidth]{res/correlation_SR_vs_IM_vivid.pdf} 
	
	\caption{Correlation between Success Rate and Ineffective Moves.
    Each model has 10 points per subplot, representing its average performance across the 10 distinct tasks (5 trials each). 
    The dashed lines indicate linear regression trends, and shaded areas represent the 95\% confidence intervals.
    }
	\label{fig:correlation}
\end{figure}

==> figs/evolved_examples.tex <==
% Examples of evolved language strategies and macro actions.
\newtcolorbox{strategybox}[1][]{
	colback=red!5!white,
	colframe=red!75!black,
	fonttitle=\bfseries,
	title=#1,
	boxrule=0.5mm,
	arc=2mm,
	left=2mm, right=2mm, top=2mm, bottom=2mm
}

\newtcolorbox{actionbox}[1][]{
	colback=orange!5!white,
	colframe=orange!75!black,
	fonttitle=\bfseries,
	title=#1,
	boxrule=0.5mm,
	arc=2mm,
	left=2mm, right=2mm, top=2mm, bottom=2mm
}

\begin{figure*}[htbp]
\centering
\begin{strategybox}[{Strategy Example 1}]
\begin{lstlisting}[breaklines=true,numbers=none]
1. Treat side-view marker sightings as coarse navigation only; only press A when the female NPC with the blue marker is front-centered from the open street side and the wall is not dominating the front view.
2. If the front view becomes wall-heavy or building-close, immediately create depth with multiple backward steps before rotating; never keep turning in place while pinned to the wall.
3. In dense NPC clusters, do not interact from a parallel wall-hugging angle. First step out toward open space, then re-approach with the marked female slightly centered and isolated from the neighboring NPC.
4. If generic ambient dialogue appears, assume wrong target or wrong angle. Finish/close it, back away, and retry from a meaningfully different street-side position rather than making tiny local corrections.
5. Once the marked female NPC is clearly engaged and dialogue has started, commit to advancing with A until the conversation ends; do not resume movement unless there is strong evidence the wrong NPC was selected.
\end{lstlisting}
\end{strategybox}
\caption{Example of an evolved language strategy for NPC interaction tasks.}
\label{fig:strategy_example_1}
\end{figure*}

\begin{figure*}[htbp]
\centering
\begin{strategybox}[{Strategy Example 2}]
\begin{lstlisting}[breaklines=true,numbers=none]
1. Use side views only to choose turning direction. If the ladder, bridge, or stairs are visible only in Left View or Right View, rotate toward that side first; do not move forward until the target is mostly in the front view.
2. At the ladder, prioritize clean front alignment over proximity. When the ladder is centered and close, press A immediately; once mounted, stop turning and chain MoveForward until the top platform is clearly reached.
3. Treat apparent open space beyond a near railing, hedge, pillar, or wall edge as suspect. If one or two forward moves produce little scene-scale change, assume a blocker, back up, rotate, and re-approach from a cleaner angle.
4. Avoid micro-oscillation near bridge and stair entrances. Once the bridge or stairs are broadly centered in front and side views are not dominated by a near wall, commit to repeated MoveForward instead of trying to perfect alignment.
5. Clear dialogue instantly with PressA, then resume route execution with a decisive action. Repeated dialogue usually means the agent is stalling in place, so prefer a larger reorientation or forward commit over small corrective turns afterward.
\end{lstlisting}
\end{strategybox}
\caption{Example of an evolved language strategy for navigation tasks with vertical traversal.}
\label{fig:strategy_example_2}
\end{figure*}

\begin{figure*}[htbp]
\centering
\begin{strategybox}[{Strategy Example 3}]
\begin{lstlisting}[breaklines=true,numbers=none]
1. Use the orange wall as a hazard boundary, not as a path to hug; if the wall dominates the front or right view, first create lateral/backup clearance before trying to advance.
2. Pass the two-barrier alley by staying centered and committing to an early wide bypass around the first obstacle cluster, rather than alternating tiny left-right corrections while already in contact.
3. When the far end looks like a close dead-end wall, assume it is a collision trap until a clear post/opening or explicit leave prompt is stably aligned; do not PressA on ambiguous close-up orange geometry.
4. If 2-3 actions produce almost no scene change, treat it as a real deadlock: back up multiple steps, rotate decisively, and reacquire the corridor from a less cramped viewpoint before moving forward again.
5. After clearing the barrier section, anchor on the leave interaction immediately; avoid drifting into the open street/plaza unless the leave transition is already confirmed.
\end{lstlisting}
\end{strategybox}
\caption{Example of an evolved language strategy for constrained corridor navigation.}
\label{fig:strategy_example_3}
\end{figure*}

\begin{figure*}[htbp]
\centering
\begin{actionbox}[{Macro Action Example 1}]
\begin{lstlisting}[breaklines=true,numbers=none]
[1] Action_EscapeDoorframe_LeftBias
Description: Reliable escape when pressed against a wall, hedge, or left-side doorframe. Clears collision with two backward moves, then rotates left to re-approach from a new angle.
Code:
private static async Task Action_EscapeDoorframe_LeftBias()
{
    Console.WriteLine("[Action API] Macro: Escape Doorframe Left Bias");
    await Action_MoveBackward();
    await Action_MoveBackward();
    await Action_RotateLeft();
    await Action_MoveForward();
}

[2] Action_EscapeDoorframe_RightBias
Description: Reliable escape when pressed against a wall, hedge, or right-side doorframe. Clears collision with two backward moves, then rotates right to re-approach from a new angle.
Code:
private static async Task Action_EscapeDoorframe_RightBias()
{
    Console.WriteLine("[Action API] Macro: Escape Doorframe Right Bias");
    await Action_MoveBackward();
    await Action_MoveBackward();
    await Action_RotateRight();
    await Action_MoveForward();
}

[3] Action_CommitEnter_LeftFacing
Description: Use when the entrance/interior is visible to the left and the front is nearly clear. Rotates into the doorway and chains forward movement to cross the threshold instead of hesitating at the frame.
Code:
private static async Task Action_CommitEnter_LeftFacing()
{
    Console.WriteLine("[Action API] Macro: Commit Enter Left Facing");
    await Action_RotateLeft();
    await Action_MoveForward();
    await Action_MoveForward();
}

[4] Action_CommitEnter_RightFacing
Description: Use when the entrance/interior is visible to the right and the front is nearly clear. Rotates into the doorway and chains forward movement to cross the threshold cleanly.
Code:
private static async Task Action_CommitEnter_RightFacing()
{
    Console.WriteLine("[Action API] Macro: Commit Enter Right Facing");
    await Action_RotateRight();
    await Action_MoveForward();
    await Action_MoveForward();
}

[5] Action_RecenterAndTalk
Description: Final interaction macro for when the clerk is already nearly centered in front. Makes a small orientation correction, steps into interaction range, then presses A.
Code:
private static async Task Action_RecenterAndTalk()
{
    Console.WriteLine("[Action API] Macro: Recenter And Talk");
    await Action_RotateLeft();
    await Action_MoveForward();
    await Action_PressA();
}
\end{lstlisting}
\end{actionbox}
\caption{Example of evolved macro actions for NPC interaction and collision recovery.}
\label{fig:macro_action_example_1}
\end{figure*}

\begin{figure*}[htbp]
\centering
\begin{actionbox}[{Macro Action Example 2}]
\begin{lstlisting}[breaklines=true,numbers=none]
[1] Action_EscapeCorner_BackBackRotateRightAdvance
Description: Use when the front view is blocked by a bush, wall, railing, or pillar and the route seems more open to the right. This creates space before re-aiming, preventing repeated scraping in the same corner.
Code:
private static async Task Action_EscapeCorner_BackBackRotateRightAdvance()
{
    Console.WriteLine("[Action API] Macro: Escape Corner - Back Back Rotate Right Advance");
    await Action_MoveBackward();
    await Action_MoveBackward();
    await Action_RotateRight();
    await Action_MoveForward();
}

[2] Action_EscapeCorner_BackBackRotateLeftAdvance
Description: Mirror version for cases where the route is clearer to the left. Useful for rooftop railing traps and ladder-base wall entanglement.
Code:
private static async Task Action_EscapeCorner_BackBackRotateLeftAdvance()
{
    Console.WriteLine("[Action API] Macro: Escape Corner - Back Back Rotate Left Advance");
    await Action_MoveBackward();
    await Action_MoveBackward();
    await Action_RotateLeft();
    await Action_MoveForward();
}

[3] Action_LadderCenterAndInteract_RightBias
Description: Use when the ladder is near the front but slightly right-offset or when the right side suggests the ladder lane. This stabilizes approach and immediately attempts the climb.
Code:
private static async Task Action_LadderCenterAndInteract_RightBias()
{
    Console.WriteLine("[Action API] Macro: Ladder Center And Interact - Right Bias");
    await Action_RotateRight();
    await Action_MoveForward();
    await Action_PressA();
}

[4] Action_LadderCenterAndInteract_LeftBias
Description: Mirror version for when the ladder is near the front but slightly left-offset. Designed to convert a side glimpse into a centered ladder mount attempt.
Code:
private static async Task Action_LadderCenterAndInteract_LeftBias()
{
    Console.WriteLine("[Action API] Macro: Ladder Center And Interact - Left Bias");
    await Action_RotateLeft();
    await Action_MoveForward();
    await Action_PressA();
}

[5] Action_BridgeOrStairCommitForward
Description: Use when the bridge or stairs are already mostly centered in front and no close wall dominates either side. This prevents over-rotation and forces decisive progression through the route segment.
Code:
private static async Task Action_BridgeOrStairCommitForward()
{
    Console.WriteLine("[Action API] Macro: Bridge/Stair Commit Forward");
    await Action_MoveForward();
    await Action_MoveForward();
    await Action_MoveForward();
}
\end{lstlisting}
\end{actionbox}
\caption{Example of evolved macro actions for vertical traversal and corridor escape.}
\label{fig:macro_action_example_2}
\end{figure*}


==> figs/fail.tex <==
\begin{figure*}[htbp] % [t] 表示优先将图片放在页首，也可以用 [htbp] 让系统自动调整
	\centering
	% width=\textwidth 确保图片宽度占满正文宽度
	\includegraphics[width=\linewidth]{res/fail.pdf} 
	
	\caption{\textbf{Distribution of failure categories across VLMs.}
    }
	\label{fig:fail}
\end{figure*}

==> figs/four_fail.tex <==
\begin{figure*}[htbp] % [t] 表示优先将图片放在页首，也可以用 [htbp] 让系统自动调整
	\centering
	% width=\textwidth 确保图片宽度占满正文宽度
	\includegraphics[width=0.9\textwidth]{res/four_fail.pdf} 
	
	\caption{Four Failure Type Case Studies.
    }
	\label{fig:four_fail}
    \vspace{2mm}
\end{figure*}

==> figs/interface.tex <==
\begin{figure}[htbp] % [t] 表示优先将图片放在页首，也可以用 [htbp] 让系统自动调整
	\centering
	%width=\textwidth 确保图片宽度占满正文宽度
	\includegraphics[width=\linewidth]{res/interface.pdf} 
	
	\caption{\textbf{Overview Architecture of the proposed PokeGym.}
    %\textbf{Bottom:} The Ryujinx emulator supplies visual observations directly via GPU texture. 
    %The automated evaluation module tracks task progress via AOB memory scanning.
    %\textbf{Middle:} A modular interface provides configurable observation spaces (e.g., L/R views, previous frames) and flexible action execution paradigms. 
    %\textbf{Top:} The VLM agent processes visual inputs to generate responses, with an optional self-reflection module. 
    }
	\label{interface}
\end{figure}

==> figs/long.tex <==
\begin{figure*}[htbp]
    \centering
    % 请将 'long_horizon_trajectories.png' 替换为你实际的图片文件名
    \includegraphics[width=0.85\textwidth]{res/long.pdf}
    \caption{Qualitative Examples of Long-Horizon Trajectories in PokeGym.}
    \label{fig:long_horizon_trajectories}
\end{figure*}

==> figs/motivations.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
\vspace{-16ex}% 
\centering
\includegraphics[width=\textwidth]{res/motivations.pdf}
\captionof{figure}{
Building on prior work, PokeGym features complex 3D environments, raw pixels, and scalable automated evaluation.
}
\label{motivations}
\end{center}}]


\begin{comment}
\begin{strip}
    \vspace{-15ex}
    \centering
    \includegraphics[width=1.0\textwidth]{res/motivations.pdf} 
	\captionof{figure}{Advancing prior works, PokeGym features complex 3D environments, raw pixels, and scalable automated evaluation.
    }
  %\Description{Enjoying the baseball game from the third-base
  %seats. Ichiro Suzuki preparing to bat.}
  \label{motivations}
\end{strip}


\IEEEaftertitletext{%
  \vspace{-12ex}%        % 你验证有效的数值，直接沿用
  \centering
  \includegraphics[width=\textwidth]{res/motivations.pdf}
  \captionof{figure}{Advancing prior works, PokeGym features complex 3D environments, raw pixels, and scalable automated evaluation.}
  \label{motivations}
  \vspace{1ex}%
}
\end{comment}

==> figs/stacked_bar.tex <==
\begin{figure}[htbp] % [t] 表示优先将图片放在页首，也可以用 [htbp] 让系统自动调整
	\centering
	% width=\textwidth 确保图片宽度占满正文宽度
	\includegraphics[width=\linewidth]{figs/Failure_Types_Stacked_Bar.pdf} 
	
	\caption{Percentage of Failure Categories across VLMs.
    }
	\label{fig:stacked_bar}
\end{figure}

==> journal-rebuttal-cmds.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% COMMANDS FOR REBUTTAL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% first paragraph text
% *********
% We would like to thank the Reviewers and the Associate Editor for the thoughtful comments and suggestions. 
% % 
% We carefully addressed each of the points raised in the reviews, and for convenience of the Associate Editor and Reviewers, 
% we list our actions toward each one of the points below. 
% % 
% We also highlight the modifications to the text by presenting them in \textcolor{red}{red} font. 
% % 
% Please note that the reference, equations, and page numbers given in the responses are those of the new manuscript.



%% separator text
% *********
% \bigskip
% {\LARGE{\noindent Comments by the Associate Editor/Reviewer 1}}
% \bigskip
% The comments of the Associate Editor/Reviewer 1 are addressed below.

\newcounter{commentnum}

%% environment for reviewer comments
% *********
\newenvironment{revcomment}%
{\stepcounter{commentnum}\vspace{0.2in}\noindent{\bf Comment  \thecommentnum:}\begin{itshape}}%
{\end{itshape}\vspace{0.2in}\\}

%% environment for author answers
% *********
\newcounter{authcommentnum}
\newenvironment{authcomment}%
{\stepcounter{authcommentnum}%\noindent{\bf Answer  \thecommentnum:\vspace{0.05in}\\}
\noindent \setlength{\parskip}{0.0em}}%
%{\vspace{0.1in}}

%% environment for manuscript edits -- the argument is for the location in the manuscript.
% *********
\newenvironment{changes}[1]%
{\begin{quotation}\noindent[#1]}%
{\end{quotation}}

%% bibliography is for new references
%\renewcommand{\bibsection}{\section*{New References}}




\definecolor{ballblue}{rgb}{0.13, 0.67, 0.8}
\definecolor{cadmiumorange}{rgb}{0.93, 0.53, 0.18}
\definecolor{asparagus}{rgb}{0.53, 0.66, 0.42}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\gray}[1]{\textcolor{gray}{#1}}

\newcommand{\review}[1]{\textcolor{gray}{[Reviewer Comment:\@ #1]}}
%\newcommand{\reviewers}[1]{\empty}

\newcommand\Rone{\textcolor{ballblue}{\textbf{R1}}}
\newcommand\Rtwo{\textcolor{cadmiumorange}{\textbf{R2}}}
\newcommand\Rthree{\textcolor{asparagus}{\textbf{R3}}}

%\newcommand{\review}[1]{\noindent\textcolor{gray}{[Review:\@ #1]}}
% \newcommand{\question}[1]{\noindent{\textbf{#1}}}
\newcommand{\question}[1]{\bigskip\noindent\textcolor{blue}{{#1\@}}}
% \question{\red{Q7({\Rtwo})}} \textbf{Summarized question goes here} Answer goes here.

\newcommand{\TODO}[1]{\textcolor{red}{[TODO: #1]}}
\definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
\definecolor{green(ryb)}{rgb}{0.4, 0.69, 0.2}
\newcommand{\dk}[1]{\textcolor{ao(english)}{#1}}
\newcommand{\dknote}[1]{{\bfseries{\textcolor{green(ryb)}{[KD: #1]}}}}

\newcommand{\rv}[1]{\textcolor{red}{#1}}

\def\eg{\emph{e.g.~}} \def\Eg{\emph{E.g.~}}
\def\ie{\emph{i.e.~}} \def\Ie{\emph{I.e.~}}
\def\cf{\emph{cf.~}} \def\Cf{\emph{Cf.~}}
\def\etc{\emph{etc.~}} \def\vs{\emph{vs.~}}
\def\wrt{w.r.t.~} \def\dof{d.o.f.~}
\def\iid{i.i.d.~} \def\wolog{w.l.o.g.~}
\def\etal{\emph{et al.~}}

\usepackage{longtable}    % 支持跨页表格
\usepackage{makecell}     % 单元格内换行
\usepackage{xcolor}       % 颜色支持
\usepackage{colortbl}     % 表格颜色填充
\usepackage{array}        % 自定义列格式

\usepackage{tcolorbox}
\tcbuselibrary{breakable} % 支持跨页

\newcommand{\rvbox}[1]{%
    \begin{tcolorbox}[
        colback=yellow!20,       % 背景颜色
        colframe=yellow!40!black, % 边框颜色
        breakable,                % 允许跨页
        boxrule=0.5pt,            % 边框粗细
        arc=0pt,                  % 无圆角
        outer arc=0pt,
        left=10pt,                % 左侧内边距
        right=10pt,               % 右侧内边距
        top=5pt,                  % 顶部内边距
        bottom=5pt,               % 底部内边距
        boxsep=0pt,               % 内容与边框间距（默认为 0pt）
        width=\textwidth,         % 宽度与文本宽度一致
        parbox=false,
    ]
    \quad #1 % 插入缩进量
    \end{tcolorbox}%
}

\input{emoji}

==> sections/backup/1_introduction_backup.tex <==
\section{Introduction}
\label{sec:intro}
	
% Artificial intelligence has demonstrated superhuman capabilities in games like chess, shogi and Go \cite{silver2018general}.
% However, when shifting from these fully observable environments through state text to perception-rich games that require visual cues and cannot rely on game states, AI systems exhibit sub-human performance \cite{balrog,lvlm_playground}.
Artificial intelligence has demonstrated superhuman capabilities in structured games like chess, shogi and Go \cite{silver2018general}, but exhibits sub-human performance in perception-rich games that must rely on visual cues rather than game states \cite{balrog,lvlm_playground}.
%
Early agents were tested in text-based or 2D games (\eg, NetHack \cite{nethack}, Atari \cite{bellemare2013arcade}), and are now benchmarked in 3D role-playing games (RPGs) \cite{doom,cradle,lumine}. Yet these environments fall short in evaluating agents' ability to \textbf{refine their configuration across consecutive episodes of the same task within long-horizon 3D games}.
%
In such settings, an agent cannot rely on a fixed, pre-programmed policy; it must learn ``on the fly'' from its own experience, a paradigm known as \textbf{test-time learning (TTL)} \cite{evotest}.
% 


% However, realizing TTL in such complex environments is difficult. Traditional approaches like online fine-tuning or reinforcement learning (RL) are ill-suited for this rapid, in-session adaptation: they are data-inefficient, requiring millions of interaction samples to learn meaningful policies \cite{bernerdota}, and their gradient-based updates are too slow and computationally expensive for the real-time decision-making loop of a single game playthrough.
% This has spurred the development of \textbf{self-evolving agents}, which adapt their internal configuration across consecutive episodes of the same task without modifying neural weights, iteratively improving task performance by analyzing trajectory feedback \cite{reflexion,voyager}.
However, realizing TTL in such environments is difficult: online fine-tuning or reinforcement learning requires millions of interaction samples and gradient updates too slow for a single playthrough \cite{bernerdota}.
This has spurred the development of \textbf{self-evolving agents}, which adapt their internal configuration across consecutive episodes of the same task without modifying neural weights, improving task performance by analyzing trajectory feedback \cite{reflexion,voyager}.

However, existing self-evolving agent frameworks largely evolve along isolated single-modality axes: some focus on the \textbf{language modality}, evolving components like the prompts, memory, or high-level strategy \cite{reasoningbank}, others on the \textbf{action modality}, evolving the agent's tool-use capabilities or generating executable actions and code \cite{voyager,agentsquare,evotest}.
% These approaches fail to optimize the visual perception and treat different modalities as separate components, failing to address the synergistic coupling required in visually-driven games, as different modalities should mutually assist and enhance each other.
These approaches fail to optimize the visual perception and treat different modalities as separate components, whereas as distinct parts of the agent's scaffold, the modalities should coordinate and mutually enhance one another.
%
% Moreover, optimizing these multimodal components jointly poses a secondary challenge: the search space of possible configurations grows exponentially, making naive trial-and-error prohibitively expensive.
Moreover, jointly optimizing these multimodal components grows the search space of possible configurations exponentially, making naive trial-and-error prohibitively expensive.
%
% A recent line of work explores  over agent configurations in open-ended search spaces.
% Some methods select among candidates through evaluation statistics (\eg count-based bandits \cite{evotest}) or heuristics (staged evaluation gates
% \cite{darwingodel}) without predictor.
% Others introduce an LLM predictor to filter evaluated candidates \cite{agentsquare}. 
% Both types of methods share the same bottleneck: a newly generated component must
% undergo a full environment evaluation before any selection mechanism can act on it, so every candidate---promising or not---costs at least one expensive rollout.
%
Recent LLM-based evolution over configurations \cite{evotest,darwingodelmachine,agentsquare} does not mitigate this cost: a newly generated component must undergo a full environment evaluation before their selection mechanism (\eg count-based bandits \cite{evotest}, in-context LLM predictor \cite{agentsquare}) can act on it, so every candidate---promising or not---costs at least one expensive rollout.
	
To navigate such vast combinatorial spaces and avoid rolling out every candidate,surrogate-based black-box optimization is often used \cite{srinivas2012information,white2021bananas,moss2020boss}. 
% It iterates over model fitting, acquisition maximization, and updating.
It iterates a loop of model fitting, acquisition maximization, evaluation, and update.
%
% However, its search space must be fixed, with even unevaluated candidates possessing predefined coordinates used to define global kernel before optimization. 
However, its search space must be fixed, with even unevaluated candidates possessing predefined coordinates before optimization. 
% the domain, the representation, and the similarity structure induced by the kernel remain unchanged throughout the search.
%
% When it comes to the open-ended space where an LLM proposes configurations that never exist before optimization, the posteriors cannot be generalized to new structures, and the exploration items cannot measure the uncertainty of candidates without predefined coordinates.
When it comes to the open-ended space where an LLM proposes configurations that never exist before optimization, the premise breaks down: without predefined coordinates, the kernel value between a new component and anything previously evaluated is undefined, which means the surrogate's posterior---and any acquisition derived from it---cannot be computed. 
% The failure is not inaccurate prediction but undefined computation.
% In this case, the candidate distribution shifts as new bottlenecks are discovered.

% Some methods \cite{agentsquare} search over evaluated modules, and use an in-context LLM
% predictor to filter candidate combinations. However, configurations containing newly evolved components without evaluated are explicitly excluded from prediction. 
% Moving beyond fixed module libraries,
% open-ended methods \cite{evotest, adas,darwingodelmachine} let an LLM generate configurations online conditioned
% execution trajectories. 
% Yet none of them learns a performance
% predictor: every generated candidate, however unpromising, has to be
% executed in the real environment, so the search cannot discard
% unpromising candidates in advance and the evaluation budget is spent
% indiscriminately. 
% The two lines of work therefore leave a clear gap:
% no existing method predicts the performance of candidates that are
% generated open-endedly, before committing to their costly evaluation.

%
% Furthermore, the evolutionary agent frameworks face three challenges. (1) \textbf{Evaluation cost}: assessing each evolved candidate requires a full environment rollout, making the optimization prohibitively expensive. 
% (2) \textbf{Cross-modal synergy modeling}: existing methods optimize modalities in isolation. They fail to capture their synergistic effects, whereas in visually-driven environments, disparate modalities should mutually assist and enhance each other.
% % (3) \textbf{Exploration-exploitation balance}: navigating the vast combinatorial search space of possible configurations requires an efficient mechanism to balance the exploration-exploitation trade-off, a problem that simple greedy or random selection cannot solve.
% (3) \textbf{Exploration-exploitation balance}: the vast search space of configurations renders greedy ineffective; navigating it instead requires an efficient mechanism to balance the exploration-exploitation trade-off, since pure exploitation may stagnate in local optima while pure exploration wastes the scarce evaluation budget.
	
% To address these gaps, we first introduce PokeGym, a visually-driven, long-horizon benchmark built upon the 3D open-world game \pokeza. By requiring agents to navigate complex urban topologies, engage in dense human-Pokémon interactions, and execute multi-stage narrative quests, PokeGym provides a testbed for evaluating advanced spatial reasoning and multi-modal planning.
To address these gaps, we introduce \textbf{PokeGym}, a visually-driven benchmark built upon the 3D open-world game \pokeza.
% Unlike text-based games or 2D grid worlds, PokeGym requires agents to navigate complex urban topologies, engage in dense human-Pokémon interactions, and execute multi-stage narrative quests from visual observations without access to text states. It evaluates agents' ability to improve spatial reasoning and multi-modal planning by evolving their configuration across consecutive attempts of the single task.
Unlike text-based games or 2D grid worlds, PokeGym requires agents to navigate complex urban topologies, engage in dense human-Pokémon interactions, and execute multi-stage narrative quests from visual observations without access to game states. It evaluates agents' ability to improve spatial reasoning and multi-modal planning by evolving their configuration across consecutive attempts of the single task.

To tackle the challenges within PokeGym, we propose Graph-Guided Evolutionary Multimodal Agent Configuration (\textbf{G-EvoMAC}). 
%
During each round, the \textbf{LLM evolver} proposes new configurations comprising visual enhancements, language strategies, and action
macros, so the search space expands as optimization proceeds.
Optimizing over such a shifting, open-ended space requires two mechanisms that fixed-space methods do not provide: a surrogate whose representation is well-defined for arbitrarily novel candidates, and an uncertainty signal that identifies structurally unseen
candidates so that scarce evaluation budgets are spent where they are most informative.
%

We instantiate the first requirement with a \textbf{performance predictor}, which encodes each configuration as a graph---components embedded in a shared pretrained space, linked by cross-modal edges---and scores it with a GNN. 
%
The topology of the graph follows the configuration's structure, so what it learns--- the mapping from cross-modal compatibility patterns to performance---applies equally to newly generated candidates.
% The topology of the graph is determined by the structure of the configuration.
% It can generalize to new patterns, as what the predictor learns is the mapping from cross-modal compatibility patterns to performance, which applies equally to newly generated candidates.
%
For the second, we introduce a \textbf{selector} that treats the disagreement among dropout-activated sub-networks of
the predictor as the uncertainty signal and evaluates the candidate
that best trades predicted performance against its disagreement.
% 
The signal is well suited to spotting structurally novel candidates
because it depends only on how the
input graph deviates from the structures seen in training.

% It is a graph-guided framework that jointly optimizes visual perception, strategy, and action-macro set synergistically.
% In visually-driven games, frame enhancements help the model focus on task-relevant regions and strengthen visual perception under complex scene conditions. 
% To overcome the prohibitive cost of evaluation, G-EvoMAC employs a \textbf{Cross-Modal Synergy Performance Predictor}, a lightweight GNN surrogate \cite{velivckovic2017graph} that learns to estimate a configuration's performance by modeling the interactions between its multimodal components. To navigate the search space efficiently, it uses a \textbf{Disagreement-Aware Selector}, which leverages the disagreement among the predictions of the GNN's sub-networks \cite{gal2016dropout} to choose the most informative configuration to evaluate next, effectively balancing exploration and exploitation \cite{srinivas2012information}.

	
	
% Our main contributions are threefold:
Our main contributions are fourfold:
\begin{itemize}
%     \item We introduce PokeGym, a visually-driven, long-horizon benchmark built upon the 3D game \pokeza, designed to evaluate test-time learning, advanced spatial reasoning, and multi-modal planning in complex urban game ecosystems.
	    \item We introduce PokeGym, a 3D game benchmark where agents act only from visual observations, designed to evaluate agents' ability to refine their configuration across consecutive episodes of the same task.
	    \item We propose G-EvoMAC, a graph-guided framework that not only extends the adaptation space to three modalities, but also models their cross-modal synergy, making them mutually enhance when evolving.
	    % \item G-EvoMAC brings surrogate-based optimization to open-ended search spaces at test time. It identifies the most promising configurations among unseen structures, eliminating the need for exhaustive rollouts.
		\item G-EvoMAC combines a graph-encoded predictor with a selector, bringing surrogate-based optimization to open-ended search spaces while spending the evaluation budget only on the most promising candidates.
		% combining a predictor with a selector to enable optimization over the open-ended search space while spending the evaluation budget only on the most promising candidates.
	    % \item G-EvoMAC brings surrogate-based optimization to open-ended search spaces. A graph-encoded predictor keeps scoring well-defined for unseen candidates, while a selector identifies structurally unseen ones and evaluates only the most promising configuration at each round.
% 	    \item Extensive experiments on PokeGym show that G-EvoMAC achieves a 60.18\% average success rate, surpassing the strongest baseline by 11.76 points.
	    \item Extensive experiments on PokeGym show that G-EvoMAC achieves a 60.18\% average success rate, surpassing the strongest baseline by 6 points.
	%     \item We conduct extensive experiments in PokeGym to demonstrate that G-EvoMAC significantly outperforms baseline methods, validating the benefits of multi-modal co-evolution and Disagreement-Aware selection.
\end{itemize}

==> tables/action_analysis.tex <==
\begin{table}[t]
\centering
\caption{Analysis on Action Execution Paradigms. 
The environment step budget remains constant across all settings in the same task.}
\label{tab:action_paradigms}
\resizebox{\linewidth}{!}{
\begin{tabular}{l| c | rrr | rrr | rrr}
    \toprule
    \textbf{Action} & \textbf{Max} & \multicolumn{3}{c|}{\textbf{Navigation}} & \multicolumn{3}{c|}{\textbf{Interaction}} & \multicolumn{3}{c}{\textbf{Mixed}} \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
    \textbf{Paradigm}& \textbf{Act/Q} & \textbf{SR$\uparrow$} & \textbf{IM\%$\downarrow$} & \textbf{Rec\%$\uparrow$} & \textbf{SR$\uparrow$} & \textbf{IM\%$\downarrow$} & \textbf{Rec\%$\uparrow$} & \textbf{SR$\uparrow$} & \textbf{IM\%$\downarrow$} & \textbf{Rec\%$\uparrow$} \\
    \midrule

    High-level 
    & 1 & 25.00 & 25.52 & 25.66 & 40.00 & \textbf{0.65}  & 60.00 & 40.00 & 9.36  & 12.19 \\
    Actions 
    & 3 & 31.67 & \textbf{7.74}  & \textbf{41.08} & \textbf{93.33} & 3.81  & 64.44 & \textbf{51.11} & \textbf{6.88}  & \textbf{43.55} \\
    \midrule
    
    Parametric 
    & 1 & \textbf{50.00} & 45.48 & 22.02 & 66.67 & 1.09  & \textbf{82.61} & 33.33 & 18.11 & 22.02 \\
    Control
    & 3 & 15.00 & 12.93 & 27.42 & 80.00 & 4.23  & 71.11 & 40.00 & 10.19 & 37.50 \\
    
    \bottomrule
\end{tabular}
}
\end{table}

% \begin{table}[t]
% \centering
% \caption{Analysis on Action Execution Paradigms. 
% This table evaluates GPT-5.2's performance under two action paradigms (Defined High-level Actions or Parametric Control) and two execution frequencies (1 or 3 maximum actions per query, denoted as \textbf{Max Act/Q}). 
% The maximum Environment Step Budget remains constant across all settings in the same task.}
% \label{tab:action_paradigms}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l| c | rrrr | rrrr | rrrr}
%     \toprule
%     \textbf{Action} & \textbf{Max} & \multicolumn{4}{c|}{\textbf{Navigation}} & \multicolumn{4}{c|}{\textbf{Interaction}} & \multicolumn{4}{c}{\textbf{Mixed}} \\
%     \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
%     \textbf{Paradigm}& \textbf{Act/Q} & \textbf{SR$\uparrow$} & \textbf{Stp$\downarrow$} & \textbf{IM\%$\downarrow$} & \textbf{Rec\%$\uparrow$} & \textbf{SR$\uparrow$} & \textbf{Stp$\downarrow$} & \textbf{IM\%$\downarrow$} & \textbf{Rec\%$\uparrow$} & \textbf{SR$\uparrow$} & \textbf{Stp$\downarrow$} & \textbf{IM\%$\downarrow$} & \textbf{Rec\%$\uparrow$} \\
%     \midrule

%     High-level 
%     & 1 & 25.00 & \textbf{77.20} & 25.52 & 25.66 & 40.00 & 152.17& \textbf{0.65}  & 60.00 & 40.00 & 117.67& 9.36  & 12.19 \\
%     Actions 
%     & 3 & \textbf{31.67} & 101.11& \textbf{7.74}  & \textbf{41.08} & \textbf{93.33} & \textbf{68.74} & 3.81  & \textbf{64.44} & \textbf{51.11} & \textbf{104.35} & \textbf{6.88}  & \textbf{43.55} \\
%     \midrule
    
%     Parametric 
%     & 1 & 50.00 & 82.50 & 45.48 & 22.02 & 66.67 & 67.40 & 1.09  & 82.61 & 33.33 & 67.60 & 18.11 & 22.02 \\
%     Control
%     & 3 & 15.00 & 111.33& 12.93 & 27.42 & 80.00 & 46.50 & 4.23  & 71.11 & 40.00 & 99.00 & 10.19 & 37.50 \\
    
%     \bottomrule
% \end{tabular}
% }
% \end{table}

==> tables/detailed_bench_cmp.tex <==
\begin{table*}[h]
	\centering
	\renewcommand{\arraystretch}{1.4}
	\caption{Detailed Comparison between Classic Benchmarks (ALFRED, Minecraft-based, Cradle-based) and PokeGym.}
	\label{tab:detailed_bench_cmp}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{p{0.18\linewidth} | p{0.2\linewidth} | p{0.58\linewidth}}
			\toprule
			\textbf{Dimension} & \textbf{Benchmark} & \textbf{Characteristics} \\
			\midrule
			
			% ==========================================
			% Dimension 1: Environment
			% ==========================================
			\textbf{Environment \newline (Visual \& Physics)}
			& ALFRED
			& Confined 3D indoor household scenes, fixed object placements, limited interactivity, constrained environmental physics \\
			\cline{2-3}
			& Minecraft-based
			& Voxel-based visuals, orthogonal geometry, uniform textures, predictable topology \\
			\cline{2-3}
			& \textbf{PokeGym (Ours)}
			& Unconstrained 3D open world, complex topology (slopes, stairs, invisible walls), diverse biomes, dynamic lighting and shadows, dense elements (crowds, wildlife) \\
			\midrule
			
			% ==========================================
			% Dimension 2: Observation Space
			% ==========================================
			\textbf{Observation \newline Space}
			& Minecraft-based
			& Privileged-state observations, including explicit $(x, y, z)$ coordinates, text-based inventory lists, block IDs \\
			\cline{2-3}
			& \textbf{PokeGym (Ours)}
			& Pure RGB observations, zero state leakage, no privileged API access \\
			\midrule
			
			% ==========================================
			% Dimension 3: Task Structure & Progression
			% ==========================================
			\textbf{Task Structure \newline \& Progression}
			& ALFRED
			& Linear subgoal progression, household chore tasks, short-to-medium horizons, step-by-step instructions \\
			\cline{2-3}
			& Minecraft-based
			& Self-driven progression, sandbox exploration, resource gathering, recipe-based crafting, open-ended building \\
			\cline{2-3}
			& Cradle-based
			& Main-story missions, combat scenarios, open-ended tasks such as NPC following \\
			\cline{2-3}
			& \textbf{PokeGym (Ours)}
			& Quest-driven narrative progression, long-horizon spatial planning, structured navigation, specific NPC interactions, combat requirements \\
			\midrule
			
			% ==========================================
			% Dimension 4: Evaluation Methodology
			% ==========================================
			\textbf{Evaluation \newline Methodology}
			& Cradle-based
			& Human evaluation, manual task-success verification, high annotation cost, limited scalability, potential human bias \\
			\cline{2-3}
			& \textbf{PokeGym (Ours)}
			& Automated AOB memory scanning, threshold-based verification, fast evaluation, objective judgment, scalable assessment \\
			\midrule
			
			% ==========================================
			% Dimension 5: Evaluated Capabilities
			% ==========================================
			\textbf{Evaluated \newline Capabilities}
			& ALFRED
			& Visual grounding in confined domains, step-by-step instruction following, basic object manipulation \\
			\cline{2-3}
			& Minecraft-based
			& Long-horizon planning, recipe-logic reasoning, open-world survival strategies \\
			\cline{2-3}
			& Cradle-based
			& General computer control, UI interaction, zero-shot and few-shot adaptation to new software \\
			\cline{2-3}
			& \textbf{PokeGym (Ours)}
			& Autonomous exploration, long-horizon planning, fine-grained visual grounding, semantic reasoning, depth perception, 3D spatial collision recovery, multimodal integration, narrative instruction following \\
			\bottomrule
		\end{tabular}
	}
\end{table*}

==> tables/diff_bench.tex <==
\begin{table*}[t]
	\centering
	\caption{Performance comparison between external benchmarks and our proposed PokeGym. 
		External benchmark scores (\eg, MMMU-Pro, GPQA) and PokeGym results are reported as accuracy or success rates from 0 to 1, except for ``Text Arena'', which uses absolute Elo rating.
		For compactness, some benchmark names are abbreviated: VidMMMU (VideoMMMU), ScrSpot (ScreenSpot-Pro), CharXiv (CharXiv-R), HLE (Humanity's Last Exam), and SWE-V (SWE-Bench Verified).
		PokeGym is evaluated under different instruction granularities: Vis-G (Visual-Guided), Stp-G (Step-Guided), and Goal-O (Goal-Only), as well as task categories: Nav (Navigation), Int (Interaction), and Mix (Mixed).}
	\label{tab:comprehensive_benchmark}
	\resizebox{\textwidth}{!}{ % 自适应页面宽度
		\begin{tabular}{l | cccccccc | cccccc}
			\toprule
			\multirow{2}{*}{\textbf{Model}} & \multicolumn{8}{c|}{\textbf{External Benchmarks}} & \multicolumn{6}{c}{\textbf{PokeGym (Ours)}} \\
			\cmidrule{2-9} \cmidrule{10-15}
			& MMMU-Pro & VidMMMU & ScrSpot & CharXiv & HLE & GPQA & SWE-V & Arena & Vis-G & Stp-G & Goal-O & Nav & Int & Mix \\
			\midrule
			Gemini-3-Pro  & 0.81 & 0.88 & 0.73 & 0.81 & 0.46 & 0.92 & 0.76 & 1486 & 0.42 & 0.74 & 0.56 & 0.45 & 0.87 & 0.44 \\
			GPT-5.2       & 0.80 & 0.86 & 0.86 & 0.82 & 0.35 & 0.92 & 0.80 & 1440 & 0.56 & 0.54 & 0.58 & 0.32 & 0.93 & 0.51 \\
			Qwen3-VL-30B  & 0.60 & 0.69 & 0.61 & 0.49 & 0.10 & 0.70 & 0.12 & 1383 & 0.56 & 0.48 & 0.50 & 0.45 & 0.67 & 0.44 \\
			Qwen3.5-122B  & 0.77 & 0.82 & 0.70 & 0.77 & 0.48 & 0.87 & 0.72 & 1416 & 0.60 & 0.36 & 0.44 & 0.37 & 0.69 & 0.38 \\
			Qwen3.5-35B   & 0.75 & 0.80 & 0.69 & 0.78 & 0.47 & 0.84 & 0.69 & 1400 & 0.50 & 0.46 & 0.46 & 0.45 & 0.73 & 0.24 \\
			\bottomrule
		\end{tabular}
	}
    \vspace{2mm}
\end{table*}

==> tables/encoding.tex <==
\begin{table}[t]
\centering
\caption{Encoding of configuration components.}
\label{tab:encoding}
\footnotesize
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l l l}
\toprule
\textbf{Modality} & \textbf{Encoded content} & \textbf{Encoder} \\
\midrule
Language & strategy text; macro-action descriptions & SigLIP2 text transformer \\
Vision & four enhanced key-frame views & SigLIP2 NaFlex-ViT \\
\bottomrule
\end{tabular}
\end{table}


==> tables/failure_modes.tex <==
\begin{table}[htbp]
\centering
\caption{Behavioral Analysis of Successful and Failed Episodes.
Metrics: 
Ineffective Move Rate (IM\%: the percentage of decision steps with movement actions that resulted in no spatial displacement), 
Recovery Rate (Rec\%: percentage of non-IMs immediately following an IM), 
Maximum Consecutive Ineffective Moves (MaxIM), and 
Action Entropy (Ent: the Shannon entropy of actions during $\ge 3$ consecutive IMs). }
\label{tab:success_vs_failure}

\resizebox{\linewidth}{!}{
\setlength{\tabcolsep}{2pt}
\begin{tabular}{l|l | cccc | cccc}
    \toprule
    \multirow{2.5}{*}{\textbf{Category}} & \multirow{2.5}{*}{\textbf{Model}} & 
    \multicolumn{4}{c|}{\textbf{Successful Episodes}} & 
    \multicolumn{4}{c}{\textbf{Failed Episodes}} \\
    \cmidrule(lr){3-6} \cmidrule(lr){7-10}
    
    & & \textbf{IM\%}$\downarrow$ & \textbf{Rec\%}$\uparrow$ & \textbf{MaxIM}$\downarrow$ & \textbf{Ent}$\downarrow$
    & \textbf{IM\%}$\downarrow$ & \textbf{Rec\%}$\uparrow$ & \textbf{MaxIM}$\downarrow$ & \textbf{Ent}$\downarrow$ \\
    \midrule
    
    \multirow{8}{*}{\textbf{Navigation}} 
    & GLM-4.6V             & 13.66 & 34.78 & 7.47 & 0.91 & 19.76 & 23.39 & 16.24 & 1.01 \\
    & Qwen3.5-35B          & 12.85 & 26.08 & 5.78 & 0.75 & 22.16 & 11.19 & 29.52 & 1.03 \\
    & Qwen3.5-122B         & 14.40 & 22.80 & 9.55 & 0.59 & 18.91 & 17.57 & 17.92 & 0.97 \\
    & Qwen3.5-Plus         & 3.88  & \textbf{54.44} & 1.84 & 0.31 & 6.33  & 54.13 & \textbf{3.59}  & 1.28 \\
    & Qwen3-VL-30B         & 9.02  & 35.27 & 4.93 & 0.95 & 15.85 & 25.64 & 12.21 & 1.35 \\
    & Claude-Sonnet-4.6    & 6.33  & 52.58 & 2.58 & 0.71 & 6.76  & \textbf{60.04} & 3.78  & 1.16 \\
    & Gemini-3-Pro         & \textbf{2.12}  & 54.10 & \textbf{1.15} & \textbf{0.14} & \textbf{5.54}  & 41.32 & 3.76  & \textbf{0.60} \\
    & GPT-5.2              & 5.93  & 42.98 & 3.00 & 0.37 & 8.04  & 40.84 & 5.05  & 0.80 \\
    \midrule
    
    \multirow{8}{*}{\textbf{Interaction}} 
    & GLM-4.6V             & 9.22  & 34.48 & 3.54 & 0.25 & 21.25 & 27.15 & 16.00 & 1.26 \\
    & Qwen3.5-35B          & 14.20 & 42.14 & 3.94 & 0.77 & 21.28 & 29.76 & 13.50 & 1.44 \\
    & Qwen3.5-122B         & 12.38 & 43.72 & 3.32 & 0.62 & 22.25 & 24.69 & 16.57 & 1.28 \\
    & Qwen3.5-Plus         & 9.75  & 59.60 & 2.28 & 0.42 & 12.02 & 49.67 & 4.90  & 1.44 \\
    & Qwen3-VL-30B         & 12.38 & 43.53 & 3.63 & 0.75 & 19.25 & 33.86 & 10.80 & 1.48 \\
    & Claude-Sonnet-4.6    & 7.85  & 60.11 & 1.93 & 0.45 & 9.90  & \textbf{51.52} & 4.40  & 1.27 \\
    & Gemini-3-Pro         & \textbf{1.27}  & \textbf{84.21} & \textbf{0.62} & 0.04 & \textbf{3.78}  & 51.35 & \textbf{1.50}  & \textbf{0.22} \\
    & GPT-5.2              & 2.15  & 80.65 & 0.86 & \textbf{0.00} & 11.13 & 50.68 & 4.00  & 1.00 \\
    \midrule
    
    \multirow{8}{*}{\textbf{Mixed}} 
    & GLM-4.6V             & 8.79  & 45.57 & 3.85 & 0.78 & 18.89 & 17.37 & 19.40 & 1.13 \\
    & Qwen3.5-35B          & 8.99  & 51.61 & 3.09 & 0.66 & 13.47 & 31.26 & 11.38 & 1.17 \\
    & Qwen3.5-122B         & 9.00  & 44.32 & 4.82 & 0.81 & 17.91 & 21.23 & 16.71 & 1.14 \\
    & Qwen3.5-Plus         & 4.03  & 73.68 & 1.73 & 0.09 & 7.71  & 51.47 & 3.56  & 0.97 \\
    & Qwen3-VL-30B         & 7.19  & 52.33 & 3.40 & 0.65 & 11.96 & 31.24 & 11.72 & 1.18 \\
    & Claude-Sonnet-4.6    & 4.83  & 68.64 & 2.59 & 0.86 & 10.74 & 26.98 & 10.11 & 1.39 \\
    & Gemini-3-Pro         & \textbf{0.47}  & \textbf{100.00} & \textbf{0.50} & \textbf{0.00} & \textbf{2.41}  & \textbf{74.80} & \textbf{1.44}  & \textbf{0.35} \\
    & GPT-5.2              & 1.63  & 92.31 & 0.74 & \textbf{0.00} & 9.33  & 39.58 & 5.14  & 1.11 \\
    \bottomrule
\end{tabular}
}
\end{table}

==> tables/gpt5.4.tex <==
\begin{table*}[t]
\centering
%\small % 缩小整个表格的字体（如果觉得还不够小，可以改成 \footnotesize）
\renewcommand{\arraystretch}{1.1} 
\caption{Performance comparison across 3 granularity levels in extended experiments. Success Rate (SR, \%) measures the percentage of episodes that successfully complete the task. Average Environment Steps (Stp) denote the average number of environment steps in successful episodes. Bold indicates the best performance.}
\label{tab:gpt5.4}
% 删除了强制拉伸的 \resizebox，让表格恢复自然、精致的尺寸
\begin{tabular}{c|l|cc|cc|cc|cc}
\toprule
& \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{Navigation}} & \multicolumn{2}{c|}{\textbf{Interaction}} & \multicolumn{2}{c|}{\textbf{Mixed}} & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule{3-10}
& & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ \\
\midrule

% ============== Visual Guided ==============
\multirow{3}{*}{Visual-Guided} 
& GPT-5.4-nano     & \textbf{50.00} & \textbf{101.20} & 66.67 & 93.80 & 33.33 & 110.00 & 50.00 & 101.67 \\
& GPT-5.4-mini     & 30.00 & 165.67 & 73.33 & \textbf{39.73} & \textbf{46.67} & \textbf{96.71}  & 50.00 & 100.70 \\
& GPT-5.4          & 40.00 & 103.88 & \textbf{93.33} & 53.71 & \textbf{46.67} & 102.57 & \textbf{60.00} & \textbf{86.72} \\
\midrule

% ============== Step Guided ==============
\multirow{3}{*}{Step-Guided} 
& GPT-5.4-nano     & \textbf{40.00} & 89.38 & 33.33 & 80.00 & \textbf{40.00} & \textbf{95.50}  & 37.78 & 88.29 \\
& GPT-5.4-mini     & 10.00 & \textbf{67.50} & \textbf{93.33} & 55.43 & \textbf{40.00} & 109.83 & 47.78 & 77.59 \\
& GPT-5.4          & 30.00 & 79.83 & \textbf{93.33} & \textbf{49.29} & \textbf{40.00} & 97.50 & \textbf{54.44} & \textbf{75.54} \\
\midrule

% ============== Goal Only ==============
\multirow{3}{*}{Goal-Only} 
& GPT-5.4-nano     & 20.00 & \textbf{90.75}  & 46.67 & 85.14 & 0.00  & -      & 22.22 & \textbf{87.95} \\
& GPT-5.4-mini     & 10.00 & 125.50 & \textbf{86.67} & \textbf{59.62} & \textbf{26.67} & \textbf{111.75} & 41.11 & 98.96 \\
& GPT-5.4          & \textbf{50.00} & 114.60 & 73.33 & 92.45 & 13.33 & 125.00 & \textbf{45.56} & 110.68 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/interventions.tex <==
\begin{table}[t]
\centering
\caption{Ablation Study on Deadlock Intervention Strategies.
Baseline indicates no intervention.
}
\label{tab:deadlock_intervention}

\resizebox{\linewidth}{!}{
\footnotesize
\setlength{\tabcolsep}{2pt}

\begin{tabular}{l | cc | cc | cc | cc}
    \toprule
    \multirow{2.5}{*}{\textbf{\shortstack{Intervention \\ Strategy}}} & 
    \multicolumn{2}{c|}{\textbf{Navigation}} & 
    \multicolumn{2}{c|}{\textbf{Interaction}} & 
    \multicolumn{2}{c|}{\textbf{Mixed}} &
    \multicolumn{2}{c}{\textbf{Average}} \\
    
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    
     & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ 
     & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ 
     & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ 
     & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ \\
    \midrule
    
    Baseline& 31.67 & 101.11 & 93.33 & \textbf{68.74} & \textbf{51.11} & 104.35 & 58.70 & 91.40 \\
    \midrule
    Textual Feedback        & 30.00 & 95.00  & 66.67 & 72.20 & 33.33 & 110.00 & 43.33 & 92.40 \\
    Forced Back   & \textbf{40.00} & 61.88  & \textbf{100.00}& 83.40 & 46.67 & 110.86 & \textbf{62.22} & 85.38 \\
    Forced Back + Rotate    & 30.00 & \textbf{61.00}  & 86.67 & 89.23 & 33.33 & \textbf{103.40} & 50.00 & \textbf{84.54} \\
    
    \bottomrule
\end{tabular}
}
\end{table}

==> tables/leaderboard.tex <==
\begin{table*}[htbp]
\vspace{4mm}
\centering
\renewcommand{\arraystretch}{1.25}
\caption{PokeGym Leaderboard. Models are ranked by their overall success rate (average of SR across all 9 task configurations), with a random baseline included for reference. The three instruction granularities are abbreviated as Vis-G (Visual-Guided), Stp-G (Step-Guided), and Goal-O (Goal-Only).}
\label{tab:leaderboard_full}
\begin{tabular}{cl | ccc | ccc | ccc | c}
\toprule
\multirow{2}{*}{\textbf{Rank}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{Navigation}} & \multicolumn{3}{c|}{\textbf{Interaction}} & \multicolumn{3}{c|}{\textbf{Mixed}} & \multirow{2}{*}{\textbf{Overall SR}} \\
\cmidrule{3-11}
& & \textbf{Vis-G} & \textbf{Stp-G} & \textbf{Goal-O} & \textbf{Vis-G} & \textbf{Stp-G} & \textbf{Goal-O} & \textbf{Vis-G} & \textbf{Stp-G} & \textbf{Goal-O} & \\
\midrule

% 第1名
\textbf{\#1} & \textbf{Gemini-3-Pro} 
& 20.00 & \textbf{70.00} & 45.00 & 66.67 & \textbf{93.33} & \textbf{100.00} & 46.67 & \textbf{60.00} & 26.67 & \textbf{58.70} \\

% 第2名
\textbf{\#2} & \textbf{GPT-5.2} 
& 25.00 & 30.00 & 40.00 & \textbf{93.33} & 86.67 & \textbf{100.00} & \textbf{60.00} & 53.33 & \textbf{40.00} & \textbf{58.70} \\

% 第3名
\textbf{\#3} & GPT-5.4 
& 40.00 & 30.00 & 50.00 & \textbf{93.33} & \textbf{93.33} & 73.33 & 46.67 & 40.00 & 13.33 & 53.33 \\

% 第4名
\textbf{\#4} & Claude-Sonnet-4.6 
& 55.00 & 55.00 & \textbf{55.00} & 80.00 & 60.00 & 60.00 & 46.67 & \textbf{60.00} & 6.67 & 53.15 \\

% 第5名
\textbf{\#5} & Qwen3-VL-30B 
& 50.00 & 40.00 & 45.00 & 66.67 & 60.00 & 73.33 & 53.33 & 46.67 & 33.33 & 52.04 \\

% 第6名
\textbf{\#6} & Qwen3.5-122B 
& \textbf{60.00} & 25.00 & 25.00 & 66.67 & 66.67 & 73.33 & 53.33 & 20.00 & \textbf{40.00} & 47.78 \\

% 第7名
\textbf{\#7} & Qwen3.5-35B 
& 45.00 & 45.00 & 45.00 & 80.00 & 60.00 & 80.00 & 26.67 & 33.33 & 13.33 & 47.59 \\

% 第8名
\textbf{\#8} & GPT-5.4-mini 
& 30.00 & 10.00 & 10.00 & 73.33 & \textbf{93.33} & 86.67 & 46.67 & 40.00 & 26.67 & 46.30 \\

% 第9名
\textbf{\#9} & Qwen3.5-Plus 
& 55.00 & 50.00 & 50.00 & 66.67 & 53.33 & 46.67 & 26.67 & 26.67 & 20.00 & 43.89 \\

% 第10名
\textbf{\#10} & GLM-4.6V 
& 25.00 & 25.00 & 25.00 & 46.67 & 53.33 & 73.33 & \textbf{60.00} & 46.67 & 26.67 & 42.41 \\

% 第11名
\textbf{\#11} & GPT-5.4-nano 
& 50.00 & 40.00 & 20.00 & 66.67 & 33.33 & 46.67 & 33.33 & 40.00 & 0.00 & 36.67 \\

\midrule
% 随机基准 (不依赖指令词，故在相同任务下合并三列表现)
- & Random 
& \multicolumn{3}{c|}{0.00} & \multicolumn{3}{c|}{0.00} & \multicolumn{3}{c|}{6.67} & 2.22 \\

\bottomrule
\end{tabular}
\vspace{4mm}
\end{table*}

==> tables/modal.tex <==
\begin{table}[htbp]
\centering
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{1pt}
\caption{Ablation study on the three evolved modalities. Each row excludes one modality from the full configuration; complete results are provided in the appendix.}
\label{tab:ablation_modal}
\resizebox{\linewidth}{!}{%
% \newcommand{\mse}[2]{\begin{tabular}{@{}c@{}}#1\\[-5pt]{\tiny$\pm$#2}\end{tabular}}
\newcommand{\mse}[2]{\begin{tabular}{@{}c@{}}#1\\[-5pt]{\tiny$\pm$#2}\end{tabular}}
\newcommand{\msei}[2]{#1{\tiny$\pm$#2}}
\begin{tabular}{l cc cc cc cc}
\toprule
\multirow{2}{*}{\textbf{Configuration}} & \multicolumn{2}{c}{\textbf{Navigation}} & \multicolumn{2}{c}{\textbf{Interaction}} & \multicolumn{2}{c}{\textbf{Localization}} & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 & \textbf{SR$\uparrow$} & \textbf{IMR$\downarrow$} & \textbf{SR$\uparrow$} & \textbf{IMR$\downarrow$} & \textbf{SR$\uparrow$} & \textbf{IMR$\downarrow$} & \textbf{SR$\uparrow$} & \textbf{IMR$\downarrow$} \\
\midrule
% w/o Visual      & \mse{34.44}{5.94} & \mse{6.86}{1.19}  & \mse{42.67}{5.23} & \mse{7.13}{1.98}  & \mse{41.82}{5.32} & \mse{5.30}{1.01}  & \mse{39.82}{3.18} & \mse{6.52}{0.91}  \\
% w/o Strategy   & \mse{39.44}{6.25} & \mse{8.55}{1.32}  & \mse{48.00}{4.73} & \mse{10.19}{2.19} & \mse{53.94}{5.47} & \mse{7.31}{1.46}  & \mse{47.02}{3.16} & \mse{8.84}{1.05}  \\
% w/o Action      & \mse{42.78}{5.75} & \mse{8.26}{1.79}  & \mse{55.11}{4.76} & \mse{7.63}{1.65}  & \mse{52.12}{5.83} & \mse{7.57}{1.39}  & \mse{50.35}{3.12} & \mse{7.81}{0.94}  \\
% \midrule
% \textbf{GraphEvo}   & \textbf{\mse{46.11}{6.11}} & \textbf{\mse{5.72}{1.01}}  & \textbf{\mse{68.00}{3.83}} & \textbf{\mse{5.76}{0.89}}  & \textbf{\mse{64.85}{4.27}} & \textbf{\mse{5.07}{0.96}}  & \textbf{\mse{60.18}{2.87}} & \textbf{\mse{5.55}{0.54}}  \\
w/o Visual      & 34.44 & 6.86  & 42.67 & 7.13  & 41.82 & 5.30  & \msei{39.82}{3.18} & \msei{6.52}{0.91}  \\
w/o Strategy   & 39.44 & 8.55  & 48.00 & 10.19 & 53.94 & 7.31  & \msei{47.02}{3.16} & \msei{8.84}{1.05}  \\
w/o Action      & 42.78 & 8.26  & 55.11 & 7.63  & 52.12 & 7.57  & \msei{50.35}{3.12} & \msei{7.81}{0.94}  \\
\midrule
\textbf{GraphEvo}   & \textbf{46.11} & \textbf{5.72}  & \textbf{68.00} & \textbf{5.76}  & \textbf{64.85} & \textbf{5.07}  & \textbf{\msei{60.18}{2.87}} & \textbf{\msei{5.55}{0.54}}  \\
\bottomrule
\end{tabular}%
} % end resizebox
\end{table}


==> tables/self-reflection.tex <==
\begin{table}[t]
\centering
\caption{Comparison of model performance with (\textbf{w/}) and without (\textbf{w/o}) the Self-Reflection (Self-Refl.) module.}
\label{tab:ablation_reflection}

% 放宽字体大小，并在外部嵌套 resizebox 
\resizebox{\linewidth}{!}{
\footnotesize
% 调整列间距
\setlength{\tabcolsep}{2pt}

% 定义列格式：L + C + 4组(CC) | 共10列
\begin{tabular}{l | c | cc | cc | cc | cc}
    \toprule
    % === 表头行 1 ===
    \multirow{2.5}{*}{\textbf{Model}} & \multirow{2.5}{*}{\textbf{\shortstack{Self-\\Refl}}} & 
    \multicolumn{2}{c|}{\textbf{Navigation}} & 
    \multicolumn{2}{c|}{\textbf{Interaction}} & 
    \multicolumn{2}{c|}{\textbf{Mixed}} &
    \multicolumn{2}{c}{\textbf{Average}} \\
    
    % cmidrule 调整
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
    
    % === 表头行 2 ===
     & & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ 
     & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ 
     & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ 
     & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ \\
    \midrule
    
    % === Qwen3.5-Plus ===
    \multirow{2}{*}{Qwen3.5-Plus} 
     & w/o & \textbf{51.67} & \textbf{74.90} & 55.56 & 61.92 & \textbf{24.44} & 128.64 & 43.89 & \textbf{88.49} \\
     & w/  & 41.67 & 119.84 & \textbf{66.67} & \textbf{61.87} & \textbf{24.44} & \textbf{126.18} & \textbf{44.26} & 102.63 \\
    \midrule

    % === Qwen3-VL ===
    \multirow{2}{*}{Qwen3-VL} 
     & w/o & 45.00 & \textbf{85.04} & 66.67 & \textbf{68.67} & \textbf{44.44} & 134.25 & \textbf{52.04} & \textbf{95.98} \\
     & w/  & \textbf{55.00} & 110.70 & \textbf{68.89} & 75.55 & 28.89 & \textbf{111.77} & 50.93 & 99.34 \\
    \midrule
    
    % === GPT-5.2 ===
    \multirow{2}{*}{GPT-5.2} 
     & w/o & 31.67 & \textbf{101.11} & \textbf{93.33} & \textbf{68.74} & \textbf{51.11} & 104.35 & \textbf{58.70} & \textbf{91.40} \\
     & w/  & \textbf{33.33} & 109.95 & \textbf{93.33} & 84.02 & 48.89 & \textbf{83.05} & 58.52 & 92.34 \\
    \midrule
    
    % === Gemini-3-Pro ===
    \multirow{2}{*}{Gemini-3-Pro} 
     & w/o & 45.00 & 106.67 & 86.67 & \textbf{76.79} & \textbf{44.44} & 117.30 & 58.70 & 100.25 \\
     & w/  & \textbf{60.00} & \textbf{96.22} & \textbf{93.33} & 94.40 & \textbf{44.44} & \textbf{103.50} & \textbf{65.93} & \textbf{98.04} \\
    \bottomrule
\end{tabular}
}
\end{table}

==> tables/vision_ablation.tex <==
\begin{table}[t]
    \centering
    \caption{Analysis of Visual Inputs.
    }
    \label{tab:visual_ablation}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{cc|c|cc|cc|cc}
        \toprule
        % \multicolumn{2}{c|} 加上竖线，确保 Configuration 和 Image 列中间的竖线连贯
        \multicolumn{2}{c|}{\textbf{Configuration}} & \textbf{Image} & \multicolumn{2}{c|}{\textbf{Navigation}} & \multicolumn{2}{c|}{\textbf{Interaction}} & \multicolumn{2}{c}{\textbf{Mixed}} \\
        \cmidrule(lr){1-2} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
        \textbf{L/R Views} & \textbf{Vis. Refl.} & \textbf{Count} & \textbf{SR$\uparrow$} & \textbf{Stp$\downarrow$} & \textbf{SR$\uparrow$} & \textbf{Stp$\downarrow$} & \textbf{SR$\uparrow$} & \textbf{Stp$\downarrow$} \\
        \midrule
        % 1 img: removeLRRef_gpt-5.2
        $\times$ & $\times$ & 1 & 30.00 & \textbf{79.00} & 46.67 & 104.14 & 33.33 & 70.60 \\
        % 2 imgs: removeLeftRight_gpt-5.2
        $\times$ & \checkmark & 2 & \textbf{35.00} & 138.00 & 46.67 & 64.14 & \textbf{73.33} & 107.64 \\
        % 3 imgs: removeViRef_gpt-5.2
        \checkmark & $\times$ & 3 & 20.00 & 131.00 & 86.67 & \textbf{50.85} & 46.67 & \textbf{83.14} \\
        % 4 imgs: removeExp_gpt-5.2
        \checkmark & \checkmark & 4 & 31.67 & 101.11 & \textbf{93.33} & 68.74 & 51.11 & 104.35 \\
        \bottomrule
    \end{tabular}%
    } % 结束 resizebox
\end{table}

==> tables/vlm_comparsion.tex <==
\begin{table}[t]
\centering
\caption{Performance comparison across 3 granularity levels. 
Success Rate (\textbf{SR}, \%) measures the percentage of episodes that successfully complete the task.
Average Environment Steps (\textbf{Stp}) denote the average number of environment steps in successful episodes. \textbf{Bold} indicates the best performance.}
\label{tab:comprehensive_results}

% 放宽字体大小，并在外部嵌套 resizebox 
\resizebox{\linewidth}{!}{
% 调整列间距
\setlength{\tabcolsep}{2pt}

% 定义列格式：L + L + 4组(CC) | 共10列
\begin{tabular}{c | l | cc | cc | cc | cc}
    \toprule
    % === 表头行 1 ===
    \multirow{2.5}{*}{\textbf{ }} & 
    \multirow{2.5}{*}{\textbf{Model}} & 
    \multicolumn{2}{c|}{\textbf{Navigation}} & 
    \multicolumn{2}{c|}{\textbf{Interaction}} & 
    \multicolumn{2}{c|}{\textbf{Mixed}} & 
    \multicolumn{2}{c}{\textbf{Average}} \\
    % cmidrule 调整，整体右移1列
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
    
    % === 表头行 2 ===
     & & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ 
     & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ 
     & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ 
     & \textbf{SR}$\uparrow$ & \textbf{Stp}$\downarrow$ \\
    \midrule
    
    % === Section 1: Visual-Guided ===
    \multirow{8}{*}{\shortstack{Visual \\ Guided}} 
    & GLM-4.6V         & 25.00 & 123.20 & 46.67 & 58.14 & \textbf{60.00} & \textbf{74.33} & 43.89 & \textbf{85.22} \\
    & Qwen3.5-35B      & 45.00 & 124.67 & 80.00 & 61.75 & 26.67 & 84.50 & 50.56 & 90.31 \\
    & Qwen3.5-122B     & \textbf{60.00} & 124.92 & 66.67 & 67.10 & 53.33 & 101.38 & 60.00 & 97.80 \\
    & Qwen3.5-Plus     & 55.00 & \textbf{81.73} & 66.67 & 65.30 & 26.67 & 153.00 & 49.45 & 100.01 \\
    & Qwen3-VL-30B         & 50.00 & 89.10 & 66.67 & 50.20 & 53.33 & 142.25 & 56.67 & 93.85 \\
    & Claude-Sonnet-4.6& 55.00 & 124.45 & 80.00 & 81.00 & 46.67 & 131.14 & \textbf{60.56} & 112.20 \\
    & Gemini-3-Pro     & 20.00 & 120.00 & 66.67 & 61.60 & 46.67 & 134.14 & 44.45 & 105.25 \\
    & GPT-5.2          & 25.00 & 147.00 & \textbf{93.33} & \textbf{41.50} & \textbf{60.00} & 86.22 & 59.44 & 91.57 \\
    
    \midrule
    % === Section 2: Step-Guided ===
    \multirow{8}{*}{\shortstack{Step \\ Guided}} 
    & GLM-4.6V         & 25.00 & 136.80 & 53.33 & 42.13 & 46.67 & \textbf{66.29} & 41.67 & 81.74 \\
    & Qwen3.5-35B      & 45.00 & 85.56 & 60.00 & 77.56 & 33.33 & 89.40 & 46.11 & 84.17 \\
    & Qwen3.5-122B     & 25.00 & 79.40 & 66.67 & \textbf{37.10} & 20.00 & 162.33 & 37.22 & 92.94 \\
    & Qwen3.5-Plus     & 50.00 & 75.70 & 53.33 & 42.75 & 26.67 & 125.50 & 43.33 & \textbf{81.32} \\
    & Qwen3-VL-30B         & 40.00 & \textbf{73.50} & 60.00 & 60.11 & 46.67 & 115.43 & 48.89 & 83.01 \\
    & Claude-Sonnet-4.6& 55.00 & 81.73 & 60.00 & 91.22 & \textbf{60.00} & 155.33 & 58.33 & 109.43 \\
    & Gemini-3-Pro     & \textbf{70.00} & 101.86 & \textbf{93.33} & 85.29 & \textbf{60.00} & 104.89 & \textbf{74.44} & 97.34 \\
    & GPT-5.2          & 30.00 & 96.00 & 86.67 & 74.62 & 53.33 & 94.00 & 56.67 & 88.21 \\

    \midrule
    % === Section 3: Goal-Only ===
    \multirow{8}{*}{\shortstack{Goal \\ Only}} 
    & GLM-4.6V         & 25.00 & 211.40 & 73.33 & 46.73 & 26.67 & 166.00 & 41.67 & 141.38 \\
    & Qwen3.5-35B      & 45.00 & 111.56 & 80.00 & 77.92 & 13.33 & 125.00 & 46.11 & 104.82 \\
    & Qwen3.5-122B     & 25.00 & 126.20 & 73.33 & \textbf{39.64} & \textbf{40.00} & 126.17 & 46.11 & 97.33 \\
    & Qwen3.5-Plus     & 50.00 & \textbf{66.60} & 46.67 & 79.00 & 20.00 & \textbf{100.33} & 38.89 & \textbf{81.98} \\
    & Qwen3-VL-30B         & 45.00 & 90.78 & 73.33 & 92.45 & 33.33 & 147.80 & 50.55 & 110.34 \\
    & Claude-Sonnet-4.6& \textbf{55.00} & 99.73 & 60.00 & 59.78 & 6.67 & 125.00 & 40.56 & 94.84 \\
    & Gemini-3-Pro     & 45.00 & 108.22 & \textbf{100.00} & 79.00 & 26.67 & 115.75 & 57.22 & 100.99 \\
    & GPT-5.2          & 40.00 & 76.25 & \textbf{100.00} & 89.07 & \textbf{40.00} & 145.33 & \textbf{60.00} & 103.55 \\
    
    \bottomrule
\end{tabular}
}
\end{table}
